Security Considerations in AI-Robotics: A Survey of Current Methods, Challenges, and Opportunities

Robotics and Artificial Intelligence (AI) have been inextricably intertwined since their inception. Today, AI-Robotics systems have become an integral part of our daily lives, from robotic vacuum cleaners to semi-autonomous cars. These systems are built upon three fundamental architectural elements: perception, navigation and planning, and control. However, while the integration of AI-Robotics systems has enhanced the quality our lives, it has also presented a serious problem - these systems are vulnerable to security attacks. The physical components, algorithms, and data that make up AI-Robotics systems can be exploited by malicious actors, potentially leading to dire consequences. Motivated by the need to address the security concerns in AI-Robotics systems, this paper presents a comprehensive survey and taxonomy across three dimensions: attack surfaces, ethical and legal concerns, and Human-Robot Interaction (HRI) security. Our goal is to provide users, developers and other stakeholders with a holistic understanding of these areas to enhance the overall AI-Robotics system security. We begin by surveying potential attack surfaces and provide mitigating defensive strategies. We then delve into ethical issues, such as dependency and psychological impact, as well as the legal concerns regarding accountability for these systems. Besides, emerging trends such as HRI are discussed, considering privacy, integrity, safety, trustworthiness, and explainability concerns. Finally, we present our vision for future research directions in this dynamic and promising field.

==> commented_stuff_from_refs.tex <==
@article{KAPPASSOV2015195,
title = {Tactile sensing in dexterous robot hands — Review},
journal = {Robotics and Autonomous Systems},
volume = {74},
pages = {195-220},
year = {2015},
issn = {0921-8890},
doi = {https://doi.org/10.1016/j.robot.2015.07.015},
url = {https://www.sciencedirect.com/science/article/pii/S0921889015001621},
author = {Zhanat Kappassov and Juan-Antonio Corrales and Véronique Perdereau},
keywords = {Tactile sensing, Tactile sensors, Robot hands, Dexterous manipulation, Tactile sensing application, Review},
abstract = {Tactile sensing is an essential element of autonomous dexterous robot hand manipulation. It provides information about forces of interaction and surface properties at points of contact between the robot fingers and the objects. Recent advancements in robot tactile sensing led to development of many computational techniques that exploit this important sensory channel. This paper reviews current state-of-the-art of manipulation and grasping applications that involve artificial sense of touch and discusses pros and cons of each technique. The main issues of artificial tactile sensing are addressed. General requirements of a tactile sensor are briefly discussed and the main transduction technologies are analyzed. Twenty eight various tactile sensors, each integrated into a robot hand, are classified in accordance with their transduction types and applications. Previously issued reviews are focused on hardware part of tactile sensors, whereas we present an overview of algorithms and tactile feedback-based control systems that exploit signals from the sensors. The applications of these algorithms include grasp stability estimation, tactile object recognition, tactile servoing and force control. Drawing from advancements in tactile sensing technology and taking into consideration its drawbacks, this paper outlines possible new directions of research in dexterous manipulation.
IMU: IMU an abbreviation for Inertial Measurement Unit is an unit which consists of accelerometer, gyroscope and magnetometer. It is capable of measuring metrics viz. linear acceleration, angular velocity and magnetic field.
IMU used for pose estimation \cite{alatise2017}
GPS: Global Positioning System (GPS) is an unit which helps in eliciting the position and time of an object based on the data received from multiple GPS satellites
Odometry: It is an unit which uses motion sensors data to calculate the appropriate change in location of a robot.
Kalman filter: Kalman filter is an algorithm which uses sensory data to mark significant points in the local map for traversal. It is highly optimal for linear Gaussian systems. \cite{kalmanfilterpaper}

==> intro_draft.tex <==


Robotics is a multidisciplinary field of engineering that deals with the design, construction, and operation of intelligent machines called robots, capable of sensing the environment and executing tasks autonomously or through human guidance. The field has made remarkable strides in reshaping industries such as transportation, manufacturing, healthcare, agriculture, entertainment, space exploration, military, and beyond. On the other hand, Artificial Intelligence (AI) is the simulation of human intelligence processes by machines, especially computer systems. In this context, AI-Robotic systems may be referred to as \emph{integration and collaboration between AI and robotic technologies}. These systems combine AI algorithms, which enable machines to perform tasks that typically require human intelligence, with robotic platforms designed to interact with and manipulate the physical world. The recent advances in machine learning (ML) and deep learning (DL) techniques has paved the way for the development of robots with cognitive abilities to execute functions such as \emph{perception, navigation, planning}, and \emph{control}. This empowerment enables robots to perceive, learn, deduce, and make real-time decisions, closely mimicking human behaviors. With ML/DL algorithms continue to advance, the synergy with robotics propels us towards a future where robots play pivotal roles in our daily lives, offering unprecedented levels of automation, efficiency, and adaptability.

%AI has been employed in robotics for a considerable period to execute activities such as \emph{perception, navigation, planning}, and \emph{control}. However, the recent progress in Machine Learning (ML) and Deep Learning (DL) has facilitated the development of robots possessing cognitive abilities. These advancements empower robots to perceive, learn, deduce, and make real-time decisions mimicking human behaviors. With AI algorithms continuing to advance, the synergy with robotics propels us towards a future where robots play pivotal roles in our daily lives, offering unprecedented levels of automation, efficiency, and adaptability.


Due to the pervasive nature of AI-Robotic systems, it has garnered unwanted interest from malicious actors who seek to compromise these systems for financial or geopolitical gain \cite{neupane2023impacts}. 
%AI-Robotics systems are vulnerable to diverse security attacks, capable of compromising their functionality, safety, and reliability. 
Despite the advancement in security methods, these systems are still vulnerable to diverse security attacks, capable of compromising their functionality, safety, and reliability. 
%Along with all the benefits, the convergence of AI into robotics introduces new attack vectors and vulnerabilities that malicious actors exploit to cause significant disruptions and harm. 
For example, adversarial attacks, data breaches, and system manipulations can lead AI-Robotics systems to cause accidents, property damage, and even endanger human lives. Furthermore, attacks on \emph{confidentiality, privacy, integrity}, and \emph{availability} can affect trust and acceptance among users \cite{yaacoub2022robotics, us_ai_report, mittal2023ai,bertino2022security}. Therefore, understanding the security dimension of AI-Robotics systems and  familiarizing oneself with the existing methods to defend against in the event of attack holds utmost importance.

%AI-Robotics systems are an amalgamation of eclectic disciplines such as engineering, computer science, mathematics, and others. Hence, to execute safe and reliable operations, ensuring the security of each component is crucial and complex. 
The security of robotics has been an active research paradigm for a long time \cite{yaacoub2022robotics, jaitly2017security, wu2007survey, mekdad2023survey, placed2023survey, li2020survey, Lamssaggad2021ASO, narayanan2016obd_securealert, chukkapalli2020ontologies}. However, with the recent influence of AI/ML on every layer of robotics architecture emerges a fresh possibility of attack surfaces. For example, as a demonstration, hackers manipulated Tesla cars into speeding up by 50 miles per hour by subtly altering a speed limit sign on the side of a road, fooling the car’s Mobileye EyeQ3 camera system \cite{tesla_crash}. Again, in 2015, a Jeep Cherokee got remotely hacked while being driven, causing Fiat Chrysler to recall 1.4 million vehicles and pay \$105 million in fines to the National Highway Traffic and Safety Administration \cite{tcsession_mobility2022}. The vulnerability occurred due to a lack of code signing in the head unit of the car \cite{jeep_cherokee} or Electronic Control Unit (ECU), allowing the gateway chip to get reprogrammed and send instructions to vehicle components, such as the steering wheel and brakes. These incidents demonstrate the importance of security in autonomous robots and vehicular systems. Likewise, the growing cognitive capabilities of AI-Robotics systems have allowed robots to interact with humans by mimicking human behaviors. These interactions possess an emotional influence on humans, especially in child psychology. An incident like Tay Poisoning \cite{tays2019} is notable among such cases, where being directly influenced by its conversations with humans, Tay started to generate inflammatory content towards other users, requiring Microsoft to decommission Tay within 24 hours with a public apology. Therefore, the ethical and Human Robot Interaction (HRI) aspect of AI-Robotics has also become relevant for safe operations, as the psychological sphere can now be a victim of the adversary \cite{swiderska2020robots}. \todo{fairness, explainable, trustworthiness}

As AI-Robotics systems become increasingly sophisticated, versatile, and integrated into our daily lives, it also revolutionizes how we work, live, and explore the world. For example, in the domain of \emph{autonomous vehicles and transportation},  self-driving cars (Waymo \cite{waymo}), drones, and Unmanned Aerial Vehicles (UAVs) is revolutionizing the transportation systems. Similarly, in \emph{industrial automation and manufacturing processes}, to improve efficiency, productivity, and safety, collaborative robots \cite{sherwani2020collaborative} perform tasks such as assembly, welding, material handling, and quality inspection. In \emph{healthcare}, AI-Robotics systems have also demonstrated their potential in revolutionizing surgery as evidenced by Smart Tissue Autonomous Robot (STAR) \cite{leonard2014smart}, and rehabilitation processes as discussed in \cite{ai2021machine}. In \emph{agriculture}, where they assist in diverse tasks like planting, harvesting, and crop health monitoring, enabling the realization of precision agriculture, as highlighted in the research of Shamshiri et al. \cite{r2018research} and Gupta et al. \cite{gupta2020security,sontowski2020cyber}. Alongside day-to-day civilian activities, defense and military operations are equally utilizing AI-Robotics systems to improve strategic capabilities while minimizing human exposure to danger \cite{lin2008autonomous}. From autonomous surveillance drones that enhance situational awareness and warfare missions to robotic vehicles for logistics transportation and reconnaissance in hazardous environments, AI-Robotics is revolutionizing how military forces plan, execute, and adapt. \todo{considerable flow breakage in the paras, reorg like - robotics, AI, Security, security incidents, in this paper}

%Despite all these advancements, 

\begin{comment}

The pervasive nature of AI-Robotic systems, as highlighted in the preceding paragraphs, has also garnered unwanted interest from malicious actors who seek to compromise these systems for financial or geopolitical gain \cite{neupane2023impacts}. 
%AI-Robotics systems are vulnerable to diverse security attacks, capable of compromising their functionality, safety, and reliability. 
Despite the advancement in security methods, these systems are still vulnerable to diverse security attacks, capable of compromising their functionality, safety, and reliability. 
%Along with all the benefits, the convergence of AI into robotics introduces new attack vectors and vulnerabilities that malicious actors exploit to cause significant disruptions and harm. 
For example, adversarial attacks, data breaches, and system manipulations can lead AI-Robotics systems to cause accidents, property damage, and even endanger human lives. Furthermore, attacks on \emph{confidentiality, privacy, integrity}, and \emph{availability} can affect trust and acceptance among users \cite{yaacoub2022robotics, us_ai_report, mittal2023ai,bertino2022security}. Therefore, understanding the security dimension of AI-Robotics systems and  familiarizing oneself with the existing methods to defend against in the event of attack holds utmost importance.

%AI-Robotics systems are an amalgamation of eclectic disciplines such as engineering, computer science, mathematics, and others. Hence, to execute safe and reliable operations, ensuring the security of each component is crucial and complex. 
The security of robotics has been an active research paradigm for a long time \cite{yaacoub2022robotics, jaitly2017security, wu2007survey, mekdad2023survey, placed2023survey, li2020survey, Lamssaggad2021ASO, narayanan2016obd_securealert, chukkapalli2020ontologies}. However, with the recent influence of AI/ML on every layer of robotics architecture emerges a fresh possibility of attack surfaces. For example, as a demonstration, hackers manipulated Tesla cars into speeding up by 50 miles per hour by subtly altering a speed limit sign on the side of a road, fooling the car’s Mobileye EyeQ3 camera system \cite{tesla_crash}. Again, in 2015, a Jeep Cherokee got remotely hacked while being driven, causing Fiat Chrysler to recall 1.4 million vehicles and pay \$105 million in fines to the National Highway Traffic and Safety Administration \cite{tcsession_mobility2022}. The vulnerability occurred due to a lack of code signing in the head unit of the car \cite{jeep_cherokee} or Electronic Control Unit (ECU), allowing the gateway chip to get reprogrammed and send instructions to vehicle components, such as the steering wheel and brakes. These incidents demonstrate the importance of security in autonomous robots and vehicular systems. Likewise, the growing cognitive capabilities of AI-Robotics systems have allowed robots to interact with humans by mimicking human behaviors. These interactions possess an emotional influence on humans, especially in child psychology. An incident like Tay Poisoning \cite{tays2019} is notable among such cases, where being directly influenced by its conversations with humans, Tay started to generate inflammatory content towards other users, requiring Microsoft to decommission Tay within 24 hours with a public apology. Therefore, the ethical and Human Robot Interaction (HRI) aspect of AI-Robotics has also become relevant for safe operations, as the psychological sphere can now be a victim of the adversary \cite{swiderska2020robots}. \todo{fairness, explainable, trustworthiness}

\end{comment}
Hence, to draw attention to potential emerging attack surfaces and their prevention approaches, with ethical and legal concerns encircling HRI, act as a catalyst behind conducting the survey. To the best of our knowledge, this survey is the first one directed towards the security of AI/ML and HRI aspects of robotics. The major contributions of this paper are as follows: 

\hl{Need to rework on contributions based on new taxonomy and rearranged sections -Subash}
\begin{itemize}


    \item We present the intricate interplay between the physical and virtual elements within AI-Robotic systems. Through a detailed examination, we present a taxonomy of attack surfaces that manifest across the layers of a three-tier hybrid robotic architecture. \todo{confusing point, break into 2}
    \item A comprehensive survey of the current attack landscape across the layers of perception, navigation and planning, and actuators. In addition to this analysis, we present defensive strategies tailored to each layer. %\todo{inconsistency between threat and attack the rest of the paper uses attack. any other keywords? needs a consistency pass}
    \item We discuss the challenges inherent within ML models, frameworks, software and explain how the existing vulnerabilities within these tools can inadvertently contribute to undermining the integrity of the final robotic systems.
    \item We present the multifaceted exploration of the ethical and legal dimensions associated with AI-Robotics systems.  
    \item We address the intricate security issues in Human-Robot Interaction (HRI), with the focus on privacy concerns. Within this context, we recommend strategic defensive solutions that aims to mitigate potential breaches.
\end{itemize}

\noindent The remainder of the sections are as follows: Section \ref{section_architecture} provides background on robotics architecture. Section \ref{section_taxonomy} summarizes our survey and taxonomy.  %Afterward, we delve into different types of attack surfaces in Section \ref{section_attack_surfaces} and introduce penetration testing. 
Following that, we investigate on attack surfaces on various layer of robotic architecture in Section \ref{section_attack_surfaces}. Then, we discuss ethical \& legal concerns surrounding the use of AI-Robotic systems in Section \ref{section_ethical_and_legal}. Section \ref{section_HRI} discusses security studies pertaining human robot interaction. Section \ref{section_research_direction} identifies research challenges and provides future direction in developing secured robotic systems. Finally, Section \ref{section_conclusion} concludes our survey.


==> resourcer.tex <==





%#### Robot Autonomy 
%Title : Artificial Intelligence for Long-Term Robot Autonomy: A Survey
%https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8421618&casa_token=ul3EnpLnuR4AAAAA:VopbAFHZoKIwovQGhaK2al_E-OnbqaFVkLZwQ44R4HaRJJSfTNQy6V3Ekj3GpylMXTxPFnKI&tag=1


% Ethical Consideration 

%title : A Review of Future and Ethical Perspectives of Robotics and AI
%https://www.frontiersin.org/articles/10.3389/frobt.2017.00075/full

==> section_ethical_and_legal.tex <==
% Swayamjit to expand the section here
Apart from attacks on input sensors (see Section \ref{section_sensor_attack}), attack on ML models used by AI-robotic systems (see Section \ref{section_training_attack} and \ref{section_inference_attack}), and attacks on actuators (see Section \ref{section_actuator_attack}), there are also ethical and legal concerns surrounding use of AI in robotics.  behavior manipulation, opacity of AI systems, bias in decision systems, human-robot interaction, automation and employment, control of autonomous systems, and \emph{machine ethics} \cite{muller2020ethics, Roszel2021KnowYM, Borg2021ExploringTA, Smuha2019TheEA}. Aside from these concerns, it also brings forth other ethical concerns. For example, the overt reliance on autonomous agents for decision-making processes can have adverse effects on human cognitive thinking and reasoning abilities, ultimately leading to a reduction in human autonomy \cite{datteri2009ethical}.

Legal and regulatory concerns stem from the application of legal and moral theories pertaining to liability and responsibility \cite{asaro2016liability}. Consider the utilization of surgical robots in hostile military environments for procedures like ``remote robotic-assisted telesurgery’’ or ``autonomous robotic surgery’’.  In the event of an unintended event mid-surgery, where harm is inflicted upon human counterparts due to malfunctioning or attack on robot actuators, this may result in legal consequences. This prompts a discussion regarding which party should be held liable, such as the system manufacturer, software developer, the autonomous agents involved (this is difficult because as they are not legal persons), or the human operators overseeing the operation of these devices \cite{o2019legal}. 

In the subsequent section, we delve into challenges and risks that arise in the context of human-robot interaction.

The ethical concern is we should implement Ai in our operations but not let them drive the agenda for us. For instance, in healthcare systems AI-Robotics systems could be used to help physicians with their jobs but not do the operation by themselves. If an AI-Robotics system is leading a clinical operation and a clinical fault happens then who should be accounted for the mistake is also a big question – the surgeon leading the surgery process, the developer of the system or the operator of the system, or the system itself. Now that being said, legal actions cannot be made on the system as it is not human. Hence, to revoke humans from getting into any sort of trouble caution and safety should be practiced when dealing with AI-Robotics systems \cite{banks2018human}. \cite{wang2018ethical} describes the various ethical concerns on healthcare robots as anticipated and asked in the form of a questionnaire by a group of AI experts, programmers, workers, labor unions’ representatives, legislators, and other stakeholders. 

Ethical concerns of AI implication is often found in military systems where the military army professionals use AI systems to get greater speed, accuracy, efficiency, extended reach and multi-level coordination. \cite{wasilow2019artificial} uses framework to anticipate the ethical concerns of AI systems in military use beforehand so that they can act in the present to bypass the concerns. 

Advances of AI in education systems certainly has boosted the learning capabilities of the students. However, ethical concerns include putting the jobs of the teacher assistants in school at stake \cite{reiss2021use}.
